Jitter Does Matter: Adapting Gaze Estimation to New Domains

Deep neural networks have demonstrated superior performance on appearance-based gaze estimation tasks. However, due to variations in person, illuminations, and background, performance degrades dramatically when applying the model to a new domain. In this paper, we discover an interesting gaze jitter phenomenon in cross-domain gaze estimation, i.e., the gaze predictions of two similar images can be severely deviated in target domain. This is closely related to cross-domain gaze estimation tasks, but surprisingly, it has not been noticed yet previously. Therefore, we innovatively propose to utilize the gaze jitter to analyze and optimize the gaze domain adaptation task. We find that the high-frequency component (HFC) is an important factor that leads to jitter. Based on this discovery, we add high-frequency components to input images using the adversarial attack and employ contrastive learning to encourage the model to obtain similar representations between original and perturbed data, which reduces the impacts of HFC. We evaluate the proposed method on four cross-domain gaze estimation tasks, and experimental results demonstrate that it significantly reduces the gaze jitter and improves the gaze estimation performance in target domains.

==> fig/attack.tex <==
    \begin{figure}
    \begin{center}
    \includegraphics[width=\linewidth]{fig/figure2.pdf}
    \end{center}
    \caption{
    % 
    Illustration of adversarial attack. Perturbation is generated from backward propagation and added to the raw images in a pixel-wise manner. Original image and adversarial samples with $\epsilon=0.01$ and $\epsilon=0.1$ (from left to right) are shown in the blue boxes. Adversarial noise significantly disturbs the gaze predictions (red arrows).
    }
    \label{fig:attack}
    \end{figure}

==> fig/teaser.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\linewidth]{fig/teaser4.pdf}
% \includegraphics[width=\linewidth]{fig/teaser.pdf}
\end{center}
\caption{
% 
The overall architecture of the proposed framework for deploying gaze estimation in new domains.
}
\label{fig:teaser}
\end{figure}

==> tab/jitter.tex <==
\begin{table}
\caption{
% 
Local-consistency on the source and target domains.% 
} % \caption
\centering
% \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lcccc@{}}
\toprule[1.2pt]
 & $\rightarrow self$ & $\rightarrow$M & $\rightarrow$D \\
\midrule
E & \textbf{0.71} & 3.99 & 6.65 \\
G & \textbf{3.07} & 4.38 & 6.00 \\
\bottomrule[1.2pt]
\end{tabular}
\label{tab:jitter}
\end{table}

% \begin{table}
% \begin{floatrow}
% \capbtabbox{
% % \centering
% \resizebox{0.8\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lcccc@{}}
% \toprule[1.2pt]
%  & $\rightarrow self$ & $\rightarrow$M & $\rightarrow$D \\
% \midrule
% E & \textbf{0.71} & 3.99 & 6.65 \\
% G & \textbf{3.07} & 4.38 & 6.00 \\
% \bottomrule[1.2pt]
% \end{tabular}}
% \label{tab:jitter}
% }{
% \caption{
% % 
% Local-consistency on the source and target domains.% 
% } % \caption
% }
% \capbtabbox{
% % \centering
% \resizebox{1.2\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{lcccc}  
% \toprule[1.5pt]
		
% \multirow{2}{1cm}{Input} & \multicolumn{2}{c}{\underline{E$\rightarrow$M}} & \multicolumn{2}{c}{\underline{G$\rightarrow$M}} \\ 
% 		&\metric    & $acc$  & \metric & $acc$  \\ 
% \midrule[1pt] 
		
% Original	 	& 3.99 & 8.56  & 4.38 & 9.52 \\ 
% Low-freq.		& \textbf{3.87}  & \textbf{7.93}  & \textbf{4.35} & \textbf{9.02} \\
		
% 		\bottomrule[1.5pt]
% 	\end{tabular} }  
% \label{tab:low-fre}
% }{
% \caption{Local-consistency and estimation accuracy when using original or low-frequency images as input.}
% }
% \end{floatrow}
% \end{table}

% \begin{table}
% \caption{
% % 
% Local-consistency on the source and target domains.% 
% } % \caption
% \centering
% % \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lcccc@{}}
% \toprule[1.2pt]
%  & $\rightarrow self$ & $\rightarrow$M & $\rightarrow$D \\
% \midrule
% E & \textbf{0.71} & 3.99 & 6.65 \\
% G & \textbf{3.07} & 4.38 & 6.00 \\
% \bottomrule[1.2pt]
% \end{tabular}
% \label{tab:jitter}
% \end{table}

==> tab/low-fre.tex <==
\begin{table} 
\caption{Local-consistency and estimation accuracy when using original or low-frequency images as input.}
\centering
\begin{tabular}{lcccc}  
\toprule[1.5pt]
		
\multirow{2}{1cm}{Input} & \multicolumn{2}{c}{\underline{E$\rightarrow$M}} & \multicolumn{2}{c}{\underline{G$\rightarrow$M}} \\ 
		&\metric    & $acc$  & \metric & $acc$  \\ 
\midrule[1pt] 
		
Original	 	& 3.99 & 8.56  & 4.38 & 9.52 \\ 
Low-freq.		& \textbf{3.87}  & \textbf{7.93}  & \textbf{4.35} & \textbf{9.02} \\
		
		\bottomrule[1.5pt]
	\end{tabular}   
\label{tab:low-fre}
\end{table}

% \begin{table} 
% \caption{Local-consistency and estimation accuracy when using original or low-frequency images as input.}
% \centering
% \begin{tabular}{lcccc}  
% \toprule[1.5pt]
		
% \multirow{2}{1cm}{Input} & \multicolumn{2}{c}{\underline{E$\rightarrow$M}} & \multicolumn{2}{c}{\underline{G$\rightarrow$M}} \\ 
% 		&\metric    & $acc$  & \metric & $acc$  \\ 
% \midrule[1pt] 
		
% Original	 	& 3.99 & 8.56  & 4.38 & 9.52 \\ 
% Low-freq.		& \textbf{3.87}  & \textbf{7.93}  & \textbf{4.35} & \textbf{9.02} \\
		
% 		\bottomrule[1.5pt]
% 	\end{tabular}   
% \label{tab:low-fre}
% \end{table}

